Greedy Output Approximation: Towards Efficient Structured Pruning for LLMs Without Retraining

To remove redundant components of large language models (LLMs) without incurring significant computational costs, this work focuses on single-shot pruning without a retraining phase. We simplify the pruning process for Transformer-based LLMs by identifying a depth-2 pruning structure that functions independently. Additionally, we propose two inference-aware pruning criteria derived from the optimization perspective of output approximation, which outperforms traditional training-aware metrics such as gradient and Hessian. We also introduce a two-step reconstruction technique to mitigate pruning errors without model retraining. Experimental results demonstrate that our approach significantly reduces computational costs and hardware requirements while maintaining superior performance across various datasets and models.

==> src/9-misc/9-ack.tex <==
\section*{Acknowledgement}

The authors wish to thank the anonymous reviewers for their helpful comments. The authors also would like to extend their sincere gratitude to the ARC (A Root Cluster for Research into Scalable Computer Systems) at the Computer Science Department of North Carolina State University. The invaluable computing resources provided by the ARC cluster (\href{https://arcb.csc.ncsu.edu/~mueller/cluster/arc/}{https://arcb.csc.ncsu.edu/~mueller/cluster/arc/}) were instrumental in facilitating the research presented in this paper.

==> src/algo/algo1.tex <==
\begin{algorithm}[!t]
\small
\caption{Pruning Redundant Attention Heads}
\begin{algorithmic}[1]
\State \textbf{Input:} Pairwise head divergence matrix $D \in \mathbb{R}^{h \times h}$, divergence threshold $\tau$
\State \textbf{Output:} List of candidate heads for pruning $C$
\State Initialize $C = []$
\For{row $i$ \textbf{and} col $j$ \textbf{in} $D$}
    \If{$D[i][j] < \tau$ \textbf{and} $(i, j) \notin edges$ \textbf{and} $(j, i) \notin edges$ \textbf{and} $i \neq j$}
        \If{$i \notin C$ \textbf{and} $j \notin C$}
            \State $C.append(i)$
        \EndIf
    \EndIf
\EndFor
\State \textbf{Prune} $C$
\end{algorithmic}
\end{algorithm}


==> src/algo/algo2.tex <==
\begin{algorithm}[!t]
\small
\caption{Pre-pruning recovery for depth-2 module with calibration data $D$}
\begin{algorithmic}[1]
\Require Assume depth-2 module $m_i$ only has single layer for each level $W_1$ and $W_2$
\Require Collect original dense outputs $Y_1, Y_2$ across dataset $D$
% \Require Define $\hat{X}_{i}, \hat{W}_{i}, \hat{Y}_{i}$ as $l_{i}$
\Procedure{Weights Reconstruction}{$\bar{W}_1, \bar{W}_2$}
\State {\# pruned modules: \{$m_1..m_{i-1}$\}}
\State $\hat{X}_1 \gets (m_{i-1}(m_{i-2}..(m_{1}X)))$ \\
- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\State $\bar{W}_{1} \gets (\hat{X}_{1}\hat{X}_{1}^{\top})^{-1}\hat{X}_{1}^{\top}Y_{1}$\\
- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\State $Y_{1} \gets \bar{W}_{1}\hat{X}_{1}$
\State $\hat{X}_2 \gets $ post-process($Y_{1}$)\\
- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\State $\bar{W}_{2} \gets (\hat{X}_{2}\hat{X}_{2}^{\top})^{-1}\hat{X}_{2}^{\top}Y_{2}$
\EndProcedure
\end{algorithmic}
\end{algorithm}


